Natural Language Robot Programming: NLP integrated with autonomous robotic grasping

In this paper, we present a grammar-based natural language framework for robot programming, specifically for pick-and-place tasks. Our approach uses a custom dictionary of action words, designed to store together words that share meaning, allowing for easy expansion of the vocabulary by adding more action words from a lexical database. We validate our Natural Language Robot Programming (NLRP) framework through simulation and real-world experimentation, using a Franka Panda robotic arm equipped with a calibrated camera-in-hand and a microphone. Participants were asked to complete a pick-and-place task using verbal commands, which were converted into text using Google's Speech-to-Text API and processed through the NLRP framework to obtain joint space trajectories for the robot. Our results indicate that our approach has a high system usability score. The framework's dictionary can be easily extended without relying on transfer learning or large data sets. In the future, we plan to compare the presented framework with different approaches of human-assisted pick-and-place tasks via a comprehensive user study.

==> parts/grasp.tex <==
For a given object and environmental constraints, grasp planning refers to the process of finding a grasp configuration that maximises the success or quality metric by allowing a stable contact between the robot end-effector and the given object. This problem has been studied extensively and many analytical as well as data-driven methods are available which ensure successful grasp planning. In this work. we use Dexnet 2.0 - a state-of-the-art grasping framework for singulated objects on table top using parallel-jaw grippers. \cite{mahler2017dex}

Dexnet 2.0 is a synthetic dataset of 6.7 million point clouds, grasps, and analytic grasp metrics generated from thousands of 3D models (from Dex-Net 1.0) in randomized poses on a table. This dataset is used for training the Grasp Quality Convolutional Neural Network (GQCNN)- a grasp model which outputs a potential grasp pose along with its robustnes value. The Grasp Quality function takes as input a set of grasp candidates and a depth image and outputs the probability of success under uncertainty in sensing and control. The GQ-CNN framework evaluates each grasp candidate and executes the most robust grasp which is kinematically reachable and does not result in collision with the table. 

\textcolor{blue}{For grasp planning, we leverage the Cross-Entropy Method (CEM), a form of derivative free optimisation, provided by Dexnet2.0. This policy models the distribution on promising grasps using Gaussian Mixture Models (GMM) and outputs the grasp configuration with the highest robustness value.}

In studies performing the comparison between various grasping methods, Dexnet2.0 has been found to be as reliable as and 3 times faster than the Point cloud registration methods. It is found to have 99\% precision when tested on 40 novel objects. 


%The robustness of a grasp is defined as $Q(\mathbf{u}, \mathbf{y})=\mathbb{E}[S \mid \mathbf{u}, \mathbf{y}]$ where $\mathbf{u}=(\mathbf{p}, \varphi) \in \mathbb{R}^{3} \times \mathcal{S}^{1}$ denotes a parallel jaw grasp in 3D space. p is the centre of the grasp, $p =(x,y,z)$ and $\phi$ is an angle in the table plane, $\mathbf{y}=\mathbb{R}_{+}^{H \times W}$ represents a 2.5D point cloud as a depth image.%




\includegraphics[width= 8.5 cm, height = 2 cm]{images/Dexnet_performance.png}
\newline
However, because of the uncertainties involved in estimating the gripper distance from object using the depth image as well as in predicting the planar grasps, the grasp configuration provided by GQ-CNN might not always be the best choice. To address this issue, we provide the user with a set of robust grasp configurations as opposed to a single best grasp provided by Dexnet2.0. The final set of optimal grasps is chosen so that the grasps are at a minimum Euclidean distance $\epsilon$ from each other. The operator can then choose a preferred grasp via verbal command which is then executed.   
\subsection{Point Cloud segmentation}
%In order to grasp a particular object from a set of objects available in the given point cloud scene, we perform point cloud segmentation using the Euclidean clustering method.% 
Dexnet finds planar grasps directly using the CNN-based detector from the given depth image rather than performing explicit object and pose recognition. In addition to this, given a set of singulated object, it chooses to grasp the object with highest robustness value output by the GQ-CNN model. This creates a need for performing primary object segmentation external to Dexnet.  

We use the Random Sampling Consensus (RANSAC) and kd-tree clustering algorithms for performing clustering using the Point Cloud Library (PCL). The input 2.5 D pointcloud is converted into a k-dimensional binary tree which outputs clusters corresponding to the objects in the scene. The segmented pointcloud of the user selected object is then provided as an input to the grasp planner. 

\subsubsection{PCA}



==> parts/nlp.tex <==
Whereas other approaches have relied on machine learning or parsers for specialised grammars, our approach to understanding natural language commands is underpinned by a dependency parser, specifically the implementation made available by spaCy \cite{honnibal-johnson:2015:EMNLP}. Dependency parsing automatically extracts the syntactic structure of a sentence as a tree, by identifying typed binary relationships between its words \cite{jurafsky2000speech}. 

Each of these binary relationships encodes a dependency between two words: a head and its dependent (a word that modifies or specifies the head). The head of the entire sentence---typically the main verb---becomes the root of the dependency tree. Each head-dependent relationship is assigned a type, which is any of the known English grammatical functions (e.g., subject, direct object, indirect object). Head-dependent relations are thus able to capture semantic relationships (e.g., between an action and a receiver of that action).In Figure X, we show a sample sentence together with its dependency tree, as extracted by spaCy. Each of the words in the sentence appears as a node with the part-of-speech (POS) tag indicated, specifying if the word is a noun, verb, preposition, etc~Fig.~\ref{fig:dataflow}. 
% <<<<<<<<<<<Fig>>>>>>>>>>>
\begin{figure}
\centering
\includegraphics[width= 8cm, height = 5cm]{images/High_Level_System_Diagram.png}
\caption{High level diagram showing the flow of data from the client side application to the robot. }
\label{fig:dataflow}
\end{figure}
% <<<<<<<<<<<Fig>>>>>>>>>>>

% <<<<<<<<<<<Fig>>>>>>>>>>>
\begin{figure}
\centering
\includegraphics[width= 8cm, height = 5cm]{images/Low_Level_System_Diagram_.png}
\caption{Low level diagram showing the responsibilities of each component as the data goes from client to robot.}
\label{fig:client}
\end{figure}
% <<<<<<<<<<<Fig>>>>>>>>>>>

% <<<<<<<<<<<Fig>>>>>>>>>>>
\begin{figure}
\centering
\includegraphics[width= 8cm, height = 5cm]{images/SDC_diagram.png}
\caption{Diagram visualising the how the Natural Language Processing creates the format (SDC) to output the final robot action using each words tag and dependencies sourced from spaCy.}
\label{fig:sd}
\end{figure}
% <<<<<<<<<<<Fig>>>>>>>>>>>

%Need to fix the sizing of this, it is difficult to do without making it unreadable
%\includegraphics[width= 8 cm, height = 5 cm]{images/Dependency_Tree.png}

The information in the dependency tree resulting from spaCy is then expressed in the form of a spatial description clause (SDC). As mentioned in the previous section, an SDC consists of four components, namely:
\begin{itemize}
\item an event (E): the action that the robot is required to execute
\item an object (O): the item that a command is directed at (can be any other object in the world or even a part of the robot itself)
\item a place (PL): a place in the world such as a direction or the axes to move along
\item a path (PA): the extent (in terms of a specific amount) to which the action should be taken 
\end{itemize}
We note that not all four components are expressed in every command; except for event E, any of them might be unspecified. 

As a first step towards SDC generation, we firstly compiled a custom dictionary of action words used in pick-and-place tasks. This dictionary was designed to accommodate for the process of storing words with a shared meaning together using a grammar explored by Song \cite{song2004natural} in which high level words can be expanded to include those that share the same purpose.This implementation led to an easy process of expanding the vocabulary which we did using the lexical database ‘WordNet’ \cite{miller90wordnet}. In the final dictionary there are 7 categories, each with up to 17 high level words that can be expanded to store 7 additional synonyms. 

In almost all of the cases, the word at the root of the dependency tree (i.e., the main verb) is contained in our custom dictionary and becomes the event E of the SDC. However, if the identified root is not in the dictionary, we iterate through all of the words in the sentence to find a match with the dictionary, which then becomes the value for E.

Once E is identified, we iterate through each of its dependents and depending on the tag we perform a different process in order to populate the SDC. An example would be for the path where the language processor is looking for any word with the tag ‘NNS’ which will be a unit of measurement, when this is discovered it’s dependencies are used to search for another word with the tag ‘NumMod’ which will be a number. By joining these two words together we will have a number and a unit of measurement which will make up the path such as ‘30\_Centimetres’. 
A similar process is performed for both the object and place of the SDC where they are additionally compared to the dictionary to see if a word found is a synonym of one of our high level words. This high level word is then stored as the place or path.

The resulting SDC is sent to the robot controller where depending on the high level word found for the , it makes use of the other components to instruct the robot to perform the command. In real time this whole process takes seconds and allows for an easy and reactive control experience.
